ReTaKe: Reducing Temporal and Knowledge Redundancy for Long Video Understanding

Video Large Language Models (VideoLLMs) have made significant strides in video understanding but struggle with long videos due to the limitations of their backbone LLMs. Existing solutions rely on length extrapolation, which is memory-constrained, or visual token compression, which primarily leverages low-level temporal redundancy while overlooking the more effective high-level knowledge redundancy. To address this, we propose $\textbf{ReTaKe}$, a training-free method with two novel modules DPSelect and PivotKV, to jointly reduce both temporal visual redundancy and knowledge redundancy for video compression. To align with the way of human temporal perception, DPSelect identifies keyframes based on inter-frame distance peaks. To leverage LLMs' learned prior knowledge, PivotKV marks the keyframes as pivots and compress non-pivot frames by pruning low-attention tokens in their KV cache. ReTaKe enables VideoLLMs to process 8 times longer frames (up to 2048), outperforming similar-sized models by 3-5% and even rivaling much larger ones on VideoMME, MLVU, LongVideoBench, and LVBench. Moreover, by overlapping compression operations with prefilling, ReTaKe introduces only ~10% prefilling latency overhead while reducing decoding latency by ~20%. Our code is available at https://github.com/SCZwangxiao/video-ReTaKe.

==> rebuttal/efficiency.tex <==
\begin{table}[h]

% \caption{
% Efficiency analysis. TPOT means Time Per Output Token.
% }
\vspace{-1em}

\centering
\label{tab:efficiency}
\resizebox{0.8\linewidth}{!}{


\begin{tabular}{ccc}
\hline
Methods & TPOT (ms) & FLOPs (T) \\ \hline
{\color[HTML]{939393} QWen2VL-7B} & {\color[HTML]{939393} 116.7} & {\color[HTML]{939393} 3.0} \\
QWen2VL-7B+ReTaKe & 93.9 (-19\%) & 2.7  (-8\%) \\
{\color[HTML]{939393} LLaVA-Video-7B} & {\color[HTML]{939393} 58.5} & {\color[HTML]{939393} 10.4} \\
LLaVA-Video-7B+ReTaKe & 42.74 (-26\%) & 8.6  (-17\%) \\ \hline
\end{tabular}


}\vspace{-1em}
\end{table}

==> rebuttal/keyframe_comp.tex <==
% \begin{table}[h]\footnotesize

% % \vspace{-1em}
% % \caption{
% % Comparison with other keyframe extraction strategies in 256 frames with 2x compression.
% % }
% \vspace{-1em}

% \centering
% % \label{tab:keyframe_comp}
% % \resizebox{0.7\linewidth}{!}{


% \begin{tabular}{cccc}
% \hline
% Method & VideoMME & MLVU & LVBench \\ \hline
% $\mathrm{M}^2\mathrm{SM}$  & 58.0 & 61.6 & 39.7 \\
% A2Summ  & 57.6 & 60.9 & 39.8 \\
% MA-LMM  & 59.2 & 62.8 & 40.8 \\ \hline
% DPSelect & 59.5 & 63.2 & 41.4 \\ \hline
% \end{tabular}

% % }
% \end{table}

% \vspace{-1em}




% \begin{wraptable}{r}{0.9\linewidth} \footnotesize

% \centering
% % \resizebox{0.7\linewidth}{!}{

% \begin{tabular}{cccc}
% \hline
% Method & VideoMME & MLVU & LVBench \\ \hline
% $\mathrm{M}^2\mathrm{SM}$  & 58.0 & 61.6 & 39.7 \\
% A2Summ  & 57.6 & 60.9 & 39.8 \\
% MA-LMM  & 59.2 & 62.8 & 40.8 \\ \hline
% DPSelect & 59.5 & 63.2 & 41.4 \\ \hline
% \end{tabular}

% % }
% \end{wraptable}


\setlength{\columnsep}{1pt} % Adjust column margin
\begin{wrapfigure}{r}{0.55\linewidth}
\vspace{-1em}
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{cccc}
\hline
Method & VideoMME & MLVU & LVBench \\ \hline
$\mathrm{M}^2\mathrm{SM}$  & 58.0 & 61.6 & 39.7 \\
A2Summ  & 57.6 & 60.9 & 39.8 \\
MA-LMM  & 59.2 & 62.8 & 40.8 \\ \hline
DPSelect & 59.5 & 63.2 & 41.4 \\ \hline
\end{tabular}
\vspace{-1em}
\end{wrapfigure}



==> rebuttal/more_videollm.tex <==
\begin{table}[h]
% \caption{
% ReTaKe on more VideoLLM baselines.
% }
\vspace{-2em}
\centering
% \label{tab:more_videollm}
\resizebox{\linewidth}{!}{
% \begin{tabular}{cccc}
% \hline
% Method & VideoMME & MLVU & LVBench \\ \hline
% LLaVA-OneVision-7B & 58.4 & 62.3 & 39.9 \\
% LLaVA-OneVision-7B + ReTaKe & 60.2 & 64.8 & 42.9 \\
% LLaVA-Video-7B & 62.2 & 64.9 & 40.1 \\
% LLaVA-Video-7B + ReTaKe & 64.0 & 67.8 & 48.5 \\ \hline
% \end{tabular}
\begin{tabular}{cccc}
\hline
Method & VideoMME & MLVU & LVBench \\ \hline
{\color[HTML]{939393} LLaVA-Onevision-7B} & {\color[HTML]{939393} 58.4} & {\color[HTML]{939393} 62.3} & {\color[HTML]{939393} 39.9} \\
LLaVA-Onevision-7B+ReTaKe & 60.2 (+1.8) & 64.8 (+2.5) & 42.9 (+3.0) \\
{\color[HTML]{939393} LLaVA-Video-7B} & {\color[HTML]{939393} 62.2} & {\color[HTML]{939393} 64.9} & {\color[HTML]{939393} 43.1} \\
LLaVA-Video-7B+ReTaKe & 64.0 (+1.8) & 67.8 (+2.9) & 48.5  (+5.4) \\ \hline
\end{tabular}
}\vspace{-1em}
\end{table}



==> sec/3_method_new_1_24.tex <==
\section{Method}

\subsection{DPSelect} \label{sec:dpselect}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/dpselect_vis.pdf}
    \caption{Illustration of temporal compression. Distance represents cosine dis-similarity between adjacent frame features.}
    \label{fig:dpselect_illustration}
\end{figure}

To reduce temporal redundancy, DPSelect extracts keyframes from input video features \(\mathbf{M} \in \mathbb{R}^{T \times N \times d}\) containing \(T\) frames with \(N\) tokens per frame. It outputs compressed features \(\mathbf{M}' \in \mathbb{R}^{t \times N \times d}\) where \(t = \lfloor \alpha_{\text{dp}}T \rfloor\). 

First, compute inter-frame dissimilarity:
\begin{equation}
\bar{D}_i = \frac{1}{N} \sum_{j=1}^{N} \left( 1 - \cos(\mathbf{m}_{i,j}, \mathbf{m}_{i+1,j}) \right) \in \mathbb{R}^{T-1}
\end{equation}

Identify candidate positions through temporal windowing:
\begin{equation}
\mathcal{P} = \bigcup_i \arg\max_{w_i} (\bar{D}) \quad \text{where } w_i = [i-\lfloor W/2 \rfloor, i+\lfloor W/2 \rfloor]
\end{equation}

Select top-\(t\) keyframes:
\begin{equation}
\mathcal{K} = \text{top-k}(\bar{D}[\mathcal{P}], k=t) \subseteq \{1,...,T\}
\end{equation}

Generate compressed sequence and mask:
\begin{equation}
\mathbf{M}'_k = \mathbf{M}_{\mathcal{K},k,:} \in \mathbb{R}^{t \times N \times d}, \quad
\mathbf{Mask}_i = \mathbb{I}(i \in \mathcal{K}) \in \{0,1\}^T
\end{equation}

\subsection{PivotKV} \label{sec:pivotkv}

Given query and key/value cache \(\mathbf{Q}, \mathbf{K}_{\text{cache}} , \mathbf{V}_{\text{cache}} \in \mathbb{R}^{T \times h_v \times \left(N \times d\right)}\), where \(T = l_q = l_k = l_v\) is the sequence length, and compression ratio \(\alpha\):

1. Compute retention length:
\begin{equation}
\hat{N} = \lfloor \alpha_{kv} N \rfloor
\end{equation}

2. Calculate attention weights with recent context:
\begin{equation}
\mathbf{A} = \text{softmax}\left(\frac{\mathbf{Q} \cdot \mathbf{K}_{\text{cache},:,-l':,:}^\top}{\sqrt{d}}\right) \in \mathbb{R}^{ h_q \times  TN \times  TN}
\end{equation}  

3. Average across query heads and attention map:
\begin{equation}
\bar{\mathbf{a}} =  \frac{1}{TN} \sum_{i=1}^{TN}  \frac{1}{h_q} \sum_{j=1}^{h_q} \mathbf{A}_{:,i,:,:} \in \mathbb{R}^{ TN }
\end{equation}

4. Apply keyframe mask \(\mathbf{Mask} \in \{0,1\}^T\), which will be broadcasted into $ TN $ with $N$ times expanding:
\begin{equation}
\bar{\mathbf{a}} += \mathbf{Mask} \cdot \infty \in \mathbb{R}^{TN}
\end{equation}

5. Select pivotal positions within each frame:
\begin{equation}
\mathbf{I} = \text{top-k}(\bar{\mathbf{a}}, k=\alpha_{kv}N, \text{dim}=-1) \in \mathbb{R}^{T \times \alpha_{kv}N}
\end{equation}

6. Compress KV cache:
\begin{equation}
\begin{aligned}
\mathbf{K}' &= \text{gather}(\mathbf{K}_{\text{cache},:,-l':,:}, \mathbf{I}) \in \mathbb{R}^{T \times h_k \times \alpha_{kv}N \times d} \\
\mathbf{V}' &= \text{gather}(\mathbf{V}_{\text{cache},:,-l':,:}, \mathbf{I}) \in \mathbb{R}^{T \times h_v \times \alpha_{kv}N \times d}
\end{aligned}
\end{equation}


==> sec/3_method_old.tex <==
\section{Method}


\subsection{Overview}

Algorithm \autoref{alg:retake} outlines the general pipeline of our {\RETAKE} framework, including five steps: video encoding, DPSelect video compression, video-text splitting and chunking, chunked prefill, and decoding. 
%
In the DPSelect video compression step, keyframes are selected using DPSelect (\autoref{sec:dpselect}) to compress the video, reducing temporal redundancy. 
%
Similar to standard LLM pipelines described in \autoref{sec:preliminary}, chunked prefill encodes input videos and prompts, while decoding generates answers. The key difference is our use of chunked prefill to process video and text separately, which is mathematically equivalent to standard prefill~\cite{zeng_chunked_prefill_2024}. 
%
During chunked prefill, we apply PivotKV (\autoref{sec:pivotkv}) to compress the video KVCache, reducing knowledge redundancy by leveraging world knowledge in LLM.



\subsection{Preliminaries} \label{sec:preliminary}

% -------------------------------- Preliminary Section

% \section{Preliminary}

Similar to LLM, the inference process of VideoLLM consists of two phases: \textbf{prefill} and \textbf{decoding}. 
% The prefill phase processes the initial input data, computing self-attention representations for each token, while the decoding phase autoregressively generates new tokens by attending with all previously processed tokens. In the decoding phase, a mechanism known as the \textbf{KV cache} stores Key-Value (KV) pairs of previous tokens in memory, raising the inference speed by reducing redundant computations.
 % \subsubsection{Prefill Phase}
 
\paragraph{Prefill phase.} In the prefill phase, the input data $\mathbf{X} \in \mathbb{R}^{n \times d}$, where $n$ denotes the sequence length and $d$ represents the token dimensionality, is first transformed into query, key, and value vectors by multiplying $\mathbf{X}$ with query, key value matrices $\mathbf{W}_{\mathrm{Q}}$, $\mathbf{W}_{\mathrm{K}}$, and $\mathbf{W}_{\mathrm{V}}$:
\begin{equation} \label{eq:qkv_prefill}
    \mathbf{Q} = \mathbf{X} \mathbf{W}_{\mathrm{Q}}, \quad \mathbf{K} = \mathbf{X} \mathbf{W}_{\mathrm{K}}, \quad \mathbf{V} = \mathbf{X} \mathbf{W}_{\mathrm{V}}.    
\end{equation}
The attention output $\mathbf{O}$ is then calculated by applying the attention mechanism:
\begin{gather} \label{eq:attention_score}
\mathbf{A} = \mathrm{Softmax}\left(\frac{\mathbf{Q}\mathbf{K}^T + \mathbf{M}}{\sqrt{d}}\right), \quad \mathbf{O} = \mathbf{A} \mathbf{V}.
\end{gather}
Where \( \mathbf{A} \) represents the attention scores, and \( \mathbf{O} \) is the resulting output. The attention mask \( \mathbf{M} \in \mathbb{R}^{n \times n} \) is a lower triangular matrix that ensures each token can only attend to itself and previous tokens, thereby enforcing causality in the sequence. It's worth noting that {\textit{important tokens typically have higher attention scores}}~\cite{Serrano_interpretable_2019}.

To supplement, during the \textbf{prefill} phase, Key-Value pairs are computed for each token in the input sequence, resulting in matrices $\mathbf{K}$ and $\mathbf{V}$ (see Equations \ref{eq:qkv_prefill} and \ref{eq:attention_score}). These Key-Value pairs are stored as the \textbf{KV cache} and do not require recomputation in subsequent decoding steps. Instead, they are directly utilized in the attention mechanism, significantly improving computational efficiency.

% \subsubsection{KV Cache}
% During the \textbf{prefill} phase, Key-Value pairs are computed for each token in the input sequence, resulting in matrices $\mathbf{K}$ and $\mathbf{V}$ (see Equations \ref{eq:qkv_prefill} and \ref{eq:attention_score}). These Key-Value pairs are stored as the \textbf{KV cache} and do not require recomputation in subsequent decoding steps. Instead, they are directly utilized in the attention mechanism, significantly improving computational efficiency.

% In the \textbf{decoding} phase, each new token query $\mathbf{q}$ interacts with both the cached Key-Value pairs, $\mathbf{K}_{\mathrm{cache}}$ and $\mathbf{V}_{\mathrm{cache}}$, and the newly computed Key and Value vectors $\mathbf{K}$ and $\mathbf{V}$ from the current token. The attention calculation is performed by concatenating the cached and current token’s Key-Value matrices:
% \begin{equation}
% \text{Attention}(\mathbf{K}_{\mathrm{cache}} \mathbin\Vert \mathbf{K}, \mathbf{V}_{\mathrm{cache}} \mathbin\Vert \mathbf{V}, \mathbf{q}).
% \end{equation}
% In this equation, $\mathbf{K}_{\mathrm{cache}} \mathbin\Vert \mathbf{K}$ and $\mathbf{V}_{\mathrm{cache}} \mathbin\Vert \mathbf{V}$ represent the concatenation of the cached and current Key-Value matrices, with $\mathbin\Vert$ denoting the concatenation operation. By leveraging the \textbf{KV cache}, redundant computations for previous tokens are avoided, allowing for more efficient access to past representations during each generation step.


\input{sec/retake_algorithm}


% \subsubsection{Decoding Phase}
\paragraph{Decoding phase.} In the decoding phase, the input is the embedding of the current token $\mathbf{x} \in \mathbb{R}^{1 \times d}$, where $d$ represents the token's dimension.  The query for the current token is computed as:
\begin{equation} \label{eq:qkv_decoding}
\begin{aligned}
      \mathbf{q} &= \mathbf{x} \mathbf{W}_{\mathrm{Q}},\\ 
      \mathbf{K} &= \mathrm{Concat}(\mathbf{K}_{\mathrm{cache}}, \mathbf{x} \mathbf{W}_{\mathrm{K}}), \\  
      \mathbf{V} &= \mathrm{Concat}(\mathbf{V}_{\mathrm{cache}}, \mathbf{x} \mathbf{W}_{\mathrm{V}}).  
\end{aligned}
\end{equation}
Where $\mathbf{q}$ represents the query for the current token, while $\mathbf{K}{\mathrm{cache}}$ and $\mathbf{V}{\mathrm{cache}}$ refer to the cached Key and Value matrices from previous tokens. The key and value vectors for the current token are concatenated with their respective cached counterparts. The attention output $\mathbf{o}$ is then computed using the following attention mechanism:

\begin{gather} \label{eq:attention_decode}
\mathbf{a} = \mathrm{Softmax}\left(\frac{\mathbf{q}\mathbf{K}^T}{\sqrt{d}}\right), \quad \mathbf{o} = \mathbf{a} \mathbf{V}.
\end{gather}
Here, $\mathbf{a}$ represents the attention scores for the current token's query $\mathbf{q}$ with respect to the concatenated key matrix $\mathbf{K}$, and $\mathbf{o}$ is the resulting output.


\subsection{DPSelect} \label{sec:dpselect}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/dpselect_vis.pdf}
    \vspace{-1em}
    \caption{    
    Illustration of DPSelect. Distance represents cosine dis-similarity between the $i$-th and $i+1$-th frames.
    }
    \label{fig:dpselect_illustration}
    \vspace{-1em}
\end{figure}

To reduce low-level temporal redundancy,  DPSelect is proposed to extract keyframes based on vision encoder features, as illustrated in \autoref{fig:dpselect_illustration}. Given a long sequence of input video features \( \mathbf{M} \in \mathbb{R}^{ T \times N \times C} \) containing \(T\) frames, each frame consists of \(N\) tokens with dimension size of \(C\), DPSelect aims to compress it into a shorter sequence with minimal information loss \( \mathbf{M}' \in \mathbb{R}^{ t \times N \times C} \), where \( t < T \).
We first compute the mean pooled distance matrix between adjacent frame features as follows:
\begin{equation}
\bar{D}_i = \frac{1}{N} \sum_{j=1}^{N} \left( 1 - \cos(\mathbf{m}_{i,j}, \mathbf{m}_{i+1,j}) \right).
\end{equation}
Then max pooling is used to identify local maxima positions as candidate keyframes \( \mathcal{P} \), which is closely aligned with human video perception:
\begin{equation}
\mathcal{P} = \arg\max_{w_i} (\bar{D}_{w_i}), \quad w_i = [i-\lfloor W/2 \rfloor, i+\lfloor W/2 \rfloor],
\end{equation}
where W is the window size of max pooling. Then we filter out the final keyframes \( \mathcal{K} \) such that the compressed number of time steps does not exceed \( t \):
\begin{equation}
\mathcal{K} = \text{top-k}(\bar{D}[p], k=t).
\end{equation}
Finally, we extract the new video sequence \( \mathbf{M}' \) and corresponding mask \( \mathbf{Mask} \) based on the selected keyframes:
\begin{equation}
\mathbf{M}'_k = \mathbf{M}_{\mathcal{K},k}, \quad \forall k \in [1,N]
\end{equation}
\begin{equation}
\mathbf{Mask}_k = 
\begin{cases} 
1 & \text{if } k \in \mathcal{K} \\
0 & \text{otherwise}
\end{cases}
\end{equation}


\subsection{PivotKV} \label{sec:pivotkv}

% 通过DPSelect，我们通过模拟人类认知活动得到了关键帧，并用Mask标记出来，M接下来将会基于选中的关键帧和注意力机制进行进一步的压缩

% Given query states \( \mathbf{Q} \in \mathbb{R}^{b \times h_q \times l_q \times d} \), key states \( \mathbf{K} \in \mathbb{R}^{b \times h_k \times l_k \times d} \), and value states \( \mathbf{V} \in \mathbb{R}^{b \times h_k \times l_v \times d} \), where \( b \) is the batch size, \( h_q \) and \( h_k \)/\( h_v \)  are the number of query heads and key/value heads, respectively, \( l_q \) and \( l_k \) are the lengths of the query and key sequences, and \( d \) is the dimension of each head. Additionally, \( \mathbf{K}_{\text{cache}} \) and \( \mathbf{V}_{\text{cache}} \) represent the key-value cache.

After DPSelect, we have keyframes by simulating human cognitive activities and the corresponding mask, \( \mathbf{M} \). Next, we feed them into PivotKV to further compress the token seqence based on the keyframes and the attention mechanism, where implicitly reflects the redundancy as identified by the MLLM's high-level multimodal knowledge.

Given the batch size \( b \), the number of query heads \( h_q \) and key/value heads \( h_k \)/\( h_v \), the lengths of the query sequence \( l_q \) and key sequence \( l_k \), and head dim \( d \). Additionally, \( \mathbf{K}_{\text{cache}} \) and \( \mathbf{V}_{\text{cache}} \) represent the key-value cache. First, we compute the number of key-value pairs to retain based on the pre-defined compression ratio \( \alpha \in [0, 1] \):\(l' = \lfloor \alpha \cdot l_q \rfloor\). 

Next, we calculate the attention weights matrix \( \mathbf{A} \in \mathbb{R}^{b \times h_q \times l_q \times l_k} \) between the query states and the most recent key states:
\begin{equation}
\mathbf{A} = \text{softmax}\left( \frac{\mathbf{Q} \cdot \mathbf{K}_{\text{cache},:,-l_q:,:}^\top}{\sqrt{d}} \right).
\end{equation}

To reduce differences across heads, we sum and average the attention weights along the head dimension:
\begin{equation}
\bar{\mathbf{a}} = \frac{1}{h_k} \sum_{i=1}^{h_k} \mathbf{A}_{0,i,:,:}
\end{equation}

After that, the mask \( \mathbf{M} \in \{0, 1\}^{h_k \times l_k} \) from DPSelect is added to the attention weights before selecting the key-value pairs to retain:
\begin{equation}
\bar{\mathbf{a}} = \bar{\mathbf{a}} + \mathbf{M} \cdot \infty.
\end{equation}
Further, we select the indices of the top-\( l' \) attention weights to retain as the new KVcache.
\begin{equation}
\mathbf{I} = \text{top-k}(\bar{\mathbf{a}}, l', \text{dim}=-1)
\end{equation}
Based on the selected indices, we can extract the corresponding key and value states from the cache:
\begin{equation}
\begin{aligned}
\mathbf{K}' &= \text{gather}(\mathbf{K}_{\text{cache},:,-l_q:,:}, \mathbf{I}) \\
\mathbf{V}' &= \text{gather}(\mathbf{V}_{\text{cache},:,-l_q:,:}, \mathbf{I})
\end{aligned}
\end{equation}
The final step updates the KV cache by retaining the uncompressed part and appending the compressed part:
\begin{equation}
\begin{aligned}
\mathbf{K}_{\text{cache},:,l_k-l_q:,:} = \mathbf{K}' \\
\mathbf{V}_{\text{cache},:,l_v-l_q:,:} = \mathbf{V}'
\end{aligned}
\end{equation}
Here, the prefill phase of the proposed {\RETAKE} has been completed. The compressed KV cache obtained from previous steps enters the decoding phase, where the final answer is generated in an autoregressive manner. 

==> sec/python_code_template.tex <==
% \begin{figure*}[ht]
% \begin{lstlisting}[language=Python, style=mypython, escapechar=|, caption=Implementation of snap-KV in pseudo PyTorch style., label={lst:pytorch}]
% def snap_kv(query_states, key_states, value_states, window_size, max_capacity_prompt, kernel_size):
%     bsz, num_heads, q_len, head_dim = query_states.shape
%     # Ensure it is the prompt phase.
%     assert key_states.shape[-2] == query_states.shape[-2]
%     if q_len < max_capacity_prompt:
%         return key_states, value_states
%     else:
%         # Compute attention weights of observing window's queries and prefix context's Keys. |\label{line:start_vote}|
%         attn_weights = compute_attn(query_states[..., -window_size:, :], key_states, attention_mask) 
%         # Sum the weight along the query dimension.
%         vote = attn_weights[..., -window_size:, :-window_size].sum(dim=-2)
%         # Apply 1D pooling for clustering.
%         pool_vote = pool1d(vote, kernel_size=kernel_size, padding=kernel_size//2, stride=1) |\label{line:pooling}|
%         # Select top-k indices based on the pooled weights to identify important positions.
%         indices = pool_vote.topk(max_capacity_prompt - window_size, dim=-1).indices
%         # Expand the indices to match the head dimension for gathering.
%         indices = indices.unsqueeze(-1).expand(-1, -1, -1, head_dim) |\label{line:end_vote}|
%         # Gather the compressed past key and value states based on the selected indices. |\label{line:start_compress}|
%         k_past_compress = key_states[..., :-window_size, :].gather(dim=2, index=indices)
%         v_past_compress = value_states[..., :-window_size, :].gather(dim=2, index=indices)
%         k_obs = key_states[..., -window_size:, :]
%         v_obs = value_states[..., -window_size:, :]
%         key_states = torch.cat([k_past_compress, k_obs], dim=2)
%         value_states = torch.cat([v_past_compress, v_obs], dim=2) |\label{line:end_compress}|
%         return key_states, value_states
% \end{lstlisting}
% \end{figure*}

==> tables/cvpr_version/mlvu_lvbench_results.tex <==
\begin{table*}[t]

\caption{
Performance comparison in MLVU \cite{zhou_mlvu_2024} and LVBench \cite{wang_lvbench_2024} benchmark. ``Size'' refers to the number of parameters in LLM only.
%
Task categories in MLVU contain \cite{wang_lvbench_2024} TR--Topic Reasoning, AR--Anomaly Recognition, NQA--Needle Question-Answering, ER--Ego Reasoning, PQA--Plot Question-Answering, AO--Action Order, and AC--Action Count.
%
Task categories in LVBench \cite{wang_lvbench_2024} contain ER--Entity Recognition, EU--Event Understanding, KIR--Key Information Retrieval, TG--Temporal Grounding, and Rea--Reasoning.
}

\centering
\label{tab:mlvu_lvbench_results}
\resizebox{\linewidth}{!}{



\begin{tabular}{ccccccccccccccccc}
\hline
                                                                      &                                 & \multicolumn{8}{c}{\textbf{MLVU}}                                                                                                                                                                                                             & \textbf{}               & \multicolumn{6}{c}{\textbf{LVBench}}                                                                                                                                                                                                                                                 \\ \cline{3-17} 
                                                                      &                                 & \multicolumn{2}{c}{Holistic}                              & \multicolumn{3}{c}{Single Detail}                                                       & \multicolumn{2}{c}{Multi Detail}                          &                             & {\color[HTML]{363636} } & {\color[HTML]{363636} }                     & {\color[HTML]{363636} }                     & {\color[HTML]{363636} }                      & {\color[HTML]{363636} }                     & {\color[HTML]{363636} }                      & {\color[HTML]{363636} }                      \\ \cline{3-9}
\multirow{-3}{*}{\textbf{Methods}}                                    & \multirow{-3}{*}{\textbf{Size}} & TR                          & AR                          & NQA                         & ER                          & PQA                         & AO                          & AC                          & \multirow{-2}{*}{Avg}       & {\color[HTML]{363636} } & \multirow{-2}{*}{{\color[HTML]{363636} ER}} & \multirow{-2}{*}{{\color[HTML]{363636} EU}} & \multirow{-2}{*}{{\color[HTML]{363636} KIR}} & \multirow{-2}{*}{{\color[HTML]{363636} TG}} & \multirow{-2}{*}{{\color[HTML]{363636} Rea}} & \multirow{-2}{*}{{\color[HTML]{363636} Avg}} \\ \hline
\multicolumn{17}{c}{\textit{Proprietary Models}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
GPT-4o~\cite{openai2024gpt4o}                                         & -                               & 87.4                        & 74.5                        & 64.8                        & 57.1                        & 65.1                        & 56.7                        & 46.3                        & 64.6                        &                         & 33.0                                        & 27.4                                        & 34.5                                         & 25.0                                        & 27.5                                         & 30.8                                         \\
Gemini 1.5 Pro~\cite{Reid_Gemini1.5_2024}                             & -                               & -                           & -                           & -                           & -                           & -                           & -                           & -                           & -                           &                         & 32.1                                        & 30.9                                        & 39.3                                         & 31.8                                        & 27.0                                         & 33.1                                         \\ \hline
\multicolumn{17}{c}{\textit{Open-source Models}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
MovieChat~\cite{song2023moviechat}                                    & 7B                              & 29.5                        & 25.0                        & 24.2                        & 24.7                        & 25.8                        & 28.6                        & 22.8                        & 25.8                        &                         & 21.3                                        & 23.1                                        & 25.9                                         & 22.3                                        & 24.0                                         & 22.5                                         \\
% Movie-LLM~\cite{moviellm2024}                                         & 7B                              & 30.0                        & 29.0                        & 29.6                        & 24.7                        & 24.1                        & 20.5                        & 24.8                        & 26.1                        & \multicolumn{1}{l}{}    & -                                           & -                                           & -                                            & -                                           & -                                            & -                                            \\
TimeChat~\cite{timechat2023}                                          & 7B                              & 23.1                        & 27.0                        & 24.5                        & 28.4                        & 25.8                        & 24.7                        & 32.0                        & 30.9                        &                         & 21.9                                        & 21.7                                        & 25.9                                         & 22.7                                        & 25.0                                         & 22.3                                         \\
LLaMA-VID~\cite{li2023llama_vid}                                          & 7B                              & 50.8                        & 34.5                        & 30.1                        & 32.7                        & 32.5                        & 23.9                        & 27.8                        & 33.2                        &                         & 25.4                                        & 21.7                                        & 23.4                                         & 26.4                                        & 26.5                                         & 23.9                                         \\
Video-LLaMA2~\cite{cheng2024videollama}                              & 7B                              & 54.5                        & 41.5                        & 39.4                        & 33.5                        & 35.4                        & 18.5                        & 25.7                        & 35.5                        & \multicolumn{1}{l}{}    & -                                           & -                                           & -                                            & -                                           & -                                            & -                                            \\
MA-LMM~\cite{he_ma-lmm_2024}                                          & 7B                              & 51.9                        & 35.5                        & 43.1                        & 38.9                        & 35.8                        & 25.1                        & 24.3                        & 36.4                        & \multicolumn{1}{l}{}    & -                                           & -                                           & -                                            & -                                           & -                                            & -                                            \\
VideoChat2~\cite{Li_VideoChat2_2024}                                  & 7B                              & 74.6                        & 51.5                        & 42.0                        & 47.4                        & 43.8                        & 22.8                        & 29.6                        & 44.5                        & \multicolumn{1}{l}{}    & -                                           & -                                           & -                                            & -                                           & -                                            & -                                            \\
Video-LLaVA~\cite{lin2023videollava}                                  & 7B                              & 71.6                        & 57.0                        & 53.2                        & 45.2                        & 48.4                        & 20.1                        & 35.9                        & 47.3                        & \multicolumn{1}{l}{}    & -                                           & -                                           & -                                            & -                                           & -                                            & -                                            \\
{\color[HTML]{BFBFBF} InternVL-1.5~\cite{Chen_InternVL_2024}}         & {\color[HTML]{BFBFBF} 20B}      & {\color[HTML]{BFBFBF} 78.8} & {\color[HTML]{BFBFBF} 67.0} & {\color[HTML]{BFBFBF} 52.7} & {\color[HTML]{BFBFBF} 43.5} & {\color[HTML]{BFBFBF} 54.4} & {\color[HTML]{BFBFBF} 32.8} & {\color[HTML]{BFBFBF} 23.8} & {\color[HTML]{BFBFBF} 50.4} &                         & {\color[HTML]{BFBFBF} 37.4 }                                       & {\color[HTML]{BFBFBF} 39.7}                                        & {\color[HTML]{BFBFBF} 43.4}                                         & {\color[HTML]{BFBFBF} 31.4}                                        & {\color[HTML]{BFBFBF} 42.5}                                         & {\color[HTML]{BFBFBF} 39.6}                                         \\
{\color[HTML]{BFBFBF} VILA-1.5~\cite{xue2024longvila}}                & {\color[HTML]{BFBFBF} 40B}      & {\color[HTML]{BFBFBF} 72.8} & {\color[HTML]{BFBFBF} 59.6} & {\color[HTML]{BFBFBF} 70.6} & {\color[HTML]{BFBFBF} 53.2} & {\color[HTML]{BFBFBF} 64.7} & {\color[HTML]{BFBFBF} 42.5} & {\color[HTML]{BFBFBF} 33.4} & {\color[HTML]{BFBFBF} 56.7} &                         & -                                           & -                                           & -                                            & -                                           & -                                            & -                                            \\
CogVLM2~\cite{hong2024cogvlm2}                                        & 8B                              & -                           & -                           & -                           & -                           & -                           & -                           & -                           & -                           &                         & 28.3                                        & 27.1                                        & 31.0                                         & 25.5                                        & 25.5                                         & 28.1                                         \\
LongVA~\cite{zhang_longva_2024}                                       & 7B                              & 81.5                        & 66.6                        & 77.9                        & 60.6                        & 73.8                        & 49.3                        & 34.8                        & 63.5                        & \multicolumn{1}{l}{}    & -                                           & -                                           & -                                            & -                                           & -                                            & -                                            \\
TimeMarker~\cite{github_timemarker_2024}                              & 8B                              & 82.7                        & 65.9                        & 79.9                        & 58.7                        & 74.9                        & 49.7                        & 35.5               & 63.9                        &                         & 42.8                                        & 39.1                                        & 34.9                                         & 38.7                                        & 38.2                                         & 41.3                                         \\
Qwen2VL~\cite{wang_qwen2-vl_2024}                                    & 7B                              & 86.0                        & 62.5                        & 81.9                        & 63.6                        & 71.8                        & 53.3                        & 34.5                        & 64.8                        &                         & 44.0                                        & 41.6                                        & 43.0                                         & 39.1                                        & 43.3                                         & 42.4                                         \\
Video-XL~\cite{shu_video-xl_2024}                                     & 7B                              & 83.5                        & 68.2                        & 81.8                        & 66.2                        & 75.5                        & 48.5                        & 30.6                        & 64.9                        &                         & -                                           & -                                           & -                                            & -                                           & -                                            & -                                            \\
LLaVa-Video~\cite{zhang_llava-video_2024}                                    & 7B                              & 84.5                        & 67.0                        & 75.1                        & 59.4                        & 74.6                        & 55.6                        & 38.3                        & 64.9                        &                         & 40.5                                        & 36.3                                        & 37.5                                         & 36.8                                        & 42.3                                         & 40.1                                         \\
% 84.5,67.0,75.1,59.4,74.6,55.6,38.3,64.9,   67.0
% 40.5,36.3,37.5,36.8,42.3,36.2,40.1
{\color[HTML]{BFBFBF} LLaVA-Onevision~\cite{li_llava-onevision_2024}} & {\color[HTML]{BFBFBF} 72B}      & {\color[HTML]{BFBFBF} 84.7} & {\color[HTML]{BFBFBF} 70.6} & {\color[HTML]{BFBFBF} 82.0} & {\color[HTML]{BFBFBF} 63.1} & {\color[HTML]{BFBFBF} 75.3} & {\color[HTML]{BFBFBF} 48.7} & {\color[HTML]{BFBFBF} 40.4} & {\color[HTML]{BFBFBF} 66.4} & \multicolumn{1}{l}{}    & -                                           & -                                           & -                                            & -                                           & -                                            & -                                            \\
\textbf{Qwen2VL+\RETAKE}                                                         & 7B                              & \textbf{86.4}               & \textbf{69.0}               & \textbf{83.9}               & \textbf{73.9}               & 76.6               & 60.6               & 38.3               & \textbf{69.8}               & \textbf{}               & 49.8                               & 46.2                               & \textbf{52.9}                                & \textbf{45.0}                               & 45.8                                & 47.8                                \\
\textbf{LLaVA-Video+\RETAKE}                                                         & 7B                              & 85.6               & 67.0               & 72.5               & 65.3               & \textbf{81.3}               & \textbf{61.4}               & \textbf{41.3}               & 67.8               & \textbf{}               & \textbf{51.0}                               & \textbf{46.5}                               & 50.9                                & 42.3                               & \textbf{46.8}                                & \textbf{48.5}                                \\
{\color[HTML]{BFBFBF} Aria~\cite{li_aria_2024}}                       & {\color[HTML]{BFBFBF} 25B}      & {\color[HTML]{BFBFBF} 93.3} & {\color[HTML]{BFBFBF} 73.9} & {\color[HTML]{BFBFBF} 88.4} & {\color[HTML]{BFBFBF} 66.0} & {\color[HTML]{BFBFBF} 81.2} & {\color[HTML]{BFBFBF} 51.6} & {\color[HTML]{BFBFBF} 39.8} & {\color[HTML]{BFBFBF} 70.6} & \multicolumn{1}{l}{}    & -                                           & -                                           & -                                            & -                                           & -                                            & -                                            \\
{\color[HTML]{BFBFBF} Oryx-1.5~\cite{liu_oryx_2024}}                  & {\color[HTML]{BFBFBF} 34B}      & {\color[HTML]{BFBFBF} 89.2} & {\color[HTML]{BFBFBF} 73.5} & {\color[HTML]{BFBFBF} 84.1} & {\color[HTML]{BFBFBF} 71.7} & {\color[HTML]{BFBFBF} 77.4} & {\color[HTML]{BFBFBF} 57.7} & {\color[HTML]{BFBFBF} 52.5} & {\color[HTML]{BFBFBF} 72.3} &                         & {\color[HTML]{BFBFBF} 27.4}                                        & {\color[HTML]{BFBFBF} 29.2}                                        & {\color[HTML]{BFBFBF} 32.1}                                         & {\color[HTML]{BFBFBF} 29.1}                                        & {\color[HTML]{BFBFBF} 34.0}                                         & {\color[HTML]{BFBFBF} 30.4}                                         \\ \hline
\end{tabular}




}
\end{table*}

==> tables/cvpr_version/videomme_results.tex <==
\begin{table}[t]

\caption{
Performance comparison in VideoMME \cite{fu_videomme_2024} benchmark. ``Size'' refers to the number of parameters in LLM only. ``S'', ``M'', and ``L'' refer to the subsets of short, medium, and long duration, respectively.
}
\label{tab:videomme_results}
\centering

\resizebox{\linewidth}{!}{



\begin{tabular}{cccccc}
\hline
\textbf{Models} &
  \textbf{Size} &
  \textbf{S} &
  \textbf{M} &
  \textbf{L} &
  \textbf{Avg} \\ \hline
\multicolumn{6}{c}{\textit{Proprietary Models}} \\ \hline
{\color[HTML]{000000} GPT-4o~\cite{openai2024gpt4o}} &
  {\color[HTML]{000000} -} &
  {\color[HTML]{000000} 80.0} &
  {\color[HTML]{000000} 70.3} &
  {\color[HTML]{000000} 65.3} &
  {\color[HTML]{000000} 71.9} \\
{\color[HTML]{000000} Gemini 1.5 Pro~\cite{Reid_Gemini1.5_2024}} &
  {\color[HTML]{000000} -} &
  {\color[HTML]{000000} 81.7} &
  {\color[HTML]{000000} 74.3} &
  {\color[HTML]{000000} 67.4} &
  {\color[HTML]{000000} 75.0} \\ \hline
\multicolumn{6}{c}{\textit{Open-source Models}} \\ \hline
VideoChat2-Mistral~\cite{Li_VideoChat2_2024} &
  7B &
  48.3 &
  37.0 &
  33.2 &
  39.5 \\
ShareGPT4Video~\cite{Chen_ShareGPT4Video_2024} &
  8B &
  48.3 &
  36.3 &
  35.0 &
  39.9 \\
Video-LLaVA~\cite{lin2023videollava} &
  7B &
  45.3 &
  38.0 &
  36.2 &
  39.9 \\
SliMECASIA~\cite{Zhang_SliME_2024} &
  8B &
  53.3 &
  42.7 &
  39.8 &
  45.3 \\
LongVA~\cite{zhang_longva_2024} &
  7B &
  61.1 &
  50.4 &
  46.2 &
  52.6 \\
Long-LLaVA~\cite{Wang_LongLLaVA_2024} &
  7B &
  61.9 &
  51.4 &
  45.4 &
  52.9 \\
Kangaroo~\cite{Liu_Kangaroo_2024} &
  8B &
  66.1 &
  55.3 &
  46.6 &
  56.0 \\
VITA-1.5~\cite{fu_vita-15_2025} &
  7B &
  - &
  - &
  - &
  56.1 \\
LongVILA~\cite{xue2024longvila} &
  7B &
  69.3 &
  56.1 &
  47.0 &
  57.5 \\
% LLaVA-OneVision~\cite{li_llava-onevision_2024} &
%   7B &
%   - &
%   - &
%   - &
%   58.2 \\
{MiniCPM-V 2.6~\cite{Yao_MiniCPMV_2024}} &
  {8B} &
  {71.3} &
  {59.4} &
  {51.8} &
  {60.9} \\
{Qwen2VL~\cite{wang_qwen2-vl_2024}} &
  {7B} &
  {72.2} &
  {60.8} &
  {52.1} &
  {61.7} \\			
{LLaVA-Video～\cite{zhang_llava-video_2024}} &
  {7B} &
  {75.0} &
  {59.9} &
  {51.7} &
  {62.2} \\
{\color[HTML]{BFBFBF} InternVL2~\cite{gvlab_internvl2blog_2024}} &
  {\color[HTML]{BFBFBF} 34B} &
  {\color[HTML]{BFBFBF} 72.0} &
  {\color[HTML]{BFBFBF} 59.1} &
  {\color[HTML]{BFBFBF} 52.6} &
  {\color[HTML]{BFBFBF} 61.2} \\
{\color[HTML]{BFBFBF} VideoLLaMA 2~\cite{cheng2024videollama}} &
  {\color[HTML]{BFBFBF} 72B} &
  {\color[HTML]{BFBFBF} 69.8} &
  {\color[HTML]{BFBFBF} 59.9} &
  {\color[HTML]{BFBFBF} 57.6} &
  {\color[HTML]{BFBFBF} 62.4} \\
{\textbf{Qwen2VL+{\RETAKE}}} &
  {7B} &
  {72.8} &
  {\textbf{62.7}} &
  {\textbf{56.2}} &
  {63.9} \\
{\textbf{LLaVA-Video+{\RETAKE}}} &
  {7B} &
  {\textbf{75.0}} &
  {61.8} &
  {55.4} &
  {\textbf{64.0}} \\
% {\color[HTML]{BFBFBF} LLaVA-OneVision~\cite{li_llava-onevision_2024}} &
%   {\color[HTML]{BFBFBF} 72B} &
%   {\color[HTML]{BFBFBF} 76.7} &
%   {\color[HTML]{BFBFBF} 62.2} &
%   {\color[HTML]{BFBFBF} 60.0} &
%   {\color[HTML]{BFBFBF} 66.3} \\
{\color[HTML]{BFBFBF} LLaVA-Video~\cite{zhang_llava-video_2024}} &
  {\color[HTML]{BFBFBF} 72B} &
  {\color[HTML]{BFBFBF} 81.4} &
  {\color[HTML]{BFBFBF} 68.9} &
  {\color[HTML]{BFBFBF} 61.5} &
  {\color[HTML]{BFBFBF} 70.6} \\
{\color[HTML]{BFBFBF} Qwen2VL~\cite{wang_qwen2-vl_2024}} &
  {\color[HTML]{BFBFBF} 72B} &
  {\color[HTML]{BFBFBF} 80.1} &
  {\color[HTML]{BFBFBF} 71.3} &
  {\color[HTML]{BFBFBF} 62.2} &
  {\color[HTML]{BFBFBF} 71.2} \\ \hline
\end{tabular}


}

\end{table}
